On products of K-moduli spaces

We study the K-moduli space of products of Fano varieties in relation to the product of K-moduli spaces of the product components. We show that there exists a well-defined morphism from the product of K-moduli stacks of Fano varieties to the K-moduli stack of their product. Furthermore, we show that this morphism is an isomorphism if any two varieties with different irreducible components are non-isomorphic, and a torsor if they are. Our results rely on the theory of stacks and previous work by Zhuang. We use our main result to obtain an explicit description of the K-moduli stack/ space of Fano threefolds with Picard rank greater than 6, along with a wall-crossing description, and a detailed polyhedral wall-crossing description for K-moduli of log Fano pairs.

==> changes.tex <==
Let $X_1$, $X_2$ be two K-polystable simple $\Q$-Fano varieties. Let $A_{X_1}$ and $A_{X_2}$ be the bases of the miniversal deformations of $X_1$ and $X_2$ respectively and let $G_{X_1}$ and $G_{X_2}$ be the automorphism groups of $X_1$ and $X_2$ respectively. 
    From Theorem \ref{petracci extension-full} the base of miniversal deformations of $X=X_1\times X_2$ is $A_{X_1}\times A_{X_2}$. If $X_1\not\cong X_2$, we have $\Aut(X)\cong \Aut(X_1)\times \Aut(X_2)$. Otherwise, $\Aut(X)\cong \Aut(X_1)\times \Aut(X_2)\rtimes S_2$. The local structure of $\M^{K}_{n,V}$ is then given either by 
    $$[\operatorname{Spec}(A_{X_1})\times\operatorname{Spec}(A_{X_2})/ \Aut(X_1)\times \Aut(X_2)]\cong [\operatorname{Spec}(A_{X_1})/ \Aut(X_1)]\times[\operatorname{Spec}(A_{X_2})/ \Aut(X_2)]$$
    or
    $$[\operatorname{Spec}(A_{X_1})\times\operatorname{Spec}(A_{X_1})/ \Aut(X_1)\times \Aut(X_1)\rtimes S_2]\cong [[\operatorname{Spec}(A_{X_1})/ \Aut(X_1)^2]/S_2].$$
    In both cases, the structure may not be reduced. However, for a connected component $\M$ containing $X$
    
    
